Least Squares Regression with Markovian Data: Fundamental Limits and Algorithms

We study the problem of least squares linear regression where the data-points are dependent and are sampled from a Markov chain. We establish sharp information theoretic minimax lower bounds for this problem in terms of $\tau_{\mathsf{mix}}$, the mixing time of the underlying Markov chain, under different noise settings. Our results establish that in general, optimization with Markovian data is strictly harder than optimization with independent data and a trivial algorithm (SGD-DD) that works with only one in every $\tilde{\Theta}(\tau_{\mathsf{mix}})$ samples, which are approximately independent, is minimax optimal. In fact, it is strictly better than the popular Stochastic Gradient Descent (SGD) method with constant step-size which is otherwise minimax optimal in the regression with independent data setting. Beyond a worst case analysis, we investigate whether structured datasets seen in practice such as Gaussian auto-regressive dynamics can admit more efficient optimization schemes. Surprisingly, even in this specific and natural setting, Stochastic Gradient Descent (SGD) with constant step-size is still no better than SGD-DD. Instead, we propose an algorithm based on experience replay--a popular reinforcement learning technique--that achieves a significantly better error rate. Our improved rate serves as one of the first results where an algorithm outperforms SGD-DD on an interesting Markov chain and also provides one of the first theoretical analyses to support the use of experience replay in practice.

==> algorithms_section.tex <==
\section{Bounds for SGD and SGD-type Algorithms}
\label{sec:sgd_algs_section}
In this section, we explore advantages and limits of specific SGD algorithms in the different settings described in \ref{subsec:problem_settings}. We establish that in the agnostic setting, SGD can have a constant bias, whereas its variant, `SGD with data drop' (\sgddd) can correct this bias and is minimax optimal (up to logarithmic factors). We then consider the independent noise setting to show that SGD with constant step size (chosen independent of $\tmix$) has an extra $\tmix$ factor in the variance term. We propose a novel `Parallel SGD' algorithm that provably achieves optimal rates for regression in the independent noise case. Lastly, we provide upper and lower bounds to establish that SGD with experience replay can accelerate bias decay over standard SGD for the Gaussian Autoregressive model. This shows that under specific assumptions on the Markov chain, we can perform much better than the minimax lower bounds via. techniques like experience replay.

The specific algorithms that we analyze are variants of what we consider the ``standard" SGD algorithm with constant step size.



\begin{algorithm}
\caption{SGD with tail-averaging}
\label{alg_SGD}
\begin{algorithmic}
\REQUIRE  $T \in \mathbb{N}$ , samples $(X_1,Y_1),\dots, (X_T,Y_T) \in  \R^d\times \R$, step size $\alpha > 0$, initial point $w_1 \in \R^d$.

\FOR{t in range [1, $T$]}
\STATE  Set $w_{t+1}   \leftarrow w_t - \alpha (X_tX_t^{\intercal}w_t - X_tY_t)\,.$
\ENDFOR

\RETURN $\hat{w} \leftarrow \frac{1}{T - \lfloor T/2\rfloor}\sum_{t = \lfloor T/2\rfloor+1}^{T}w_t \,.$
\end{algorithmic}
\end{algorithm}


\vspace{5mm}

\subsection{SGD with Constant Step Size Suffers from Constant Bias in the Agnostic Setting}
\label{subsec:agnostic_SGD_bias}
It is well-known that in the i.i.d. sample setting, constant step size SGD with averaging is minimax optimal, and in particular the expected iterate $\E\left[w_t\right]$ converges to $w^*$ as $t \rightarrow \infty$. In this section we show that when the data is Markovian, and the noise in each observation $\noise_t(X)$ depends on $X$, SGD with constant step size may yield iterates that are biased estimators of the parameter $w^{*}$ even as $t \to \infty$.
%To show this, we consider $\MC_1$ and the corresponding data model defined in Section~\ref{subsec:agnostic_minimax}.  Fix a step size $\alpha > 0$. We will show that for every $\alpha \in (0,1)$, the expectation of the output of SGD is bounded away from $w_1^{*}$.  

\begin{theorem}\label{thm:agn_sgd}
	There exists a Markov chain $\MC$ with $\tmix, \kappa < C$ and global constants $c, C>0$ such that for
 	$X_0 \sim \pi(\MC)$ and $X_1 \to X_2 \to \cdots \to X_T \sim \MC$, SGD (Algorithm~\ref{alg_SGD}) run with any constant step size $\alpha>0$ leads to a constant bias, i.e., for every $t$ large enough, $$\|\mathbb{E}[w_t]-w^*\|\geq c \alpha,$$ where $w_t$ is the $t$-th step iterate of the SGD algorithm.
\end{theorem}
{\bf Remarks}:
\begin{itemize}[leftmargin=*]
	\itemsep 0pt
	\topsep 0pt
	\parskip 0pt
	\item In contrast to above result, for i.i.d. data, $\|\mathbb{E}[w_t]-w^*\|$ decreases geometrically to $0$ if $\kappa < \infty$. This also implies that the tail-averaged iterates of SGD suffer from constant bias. 
	\item The theorem is for the practically relevant case of constant step size, but geometric convergence of the bias term seems impossible even with arbitrary step sizes. We leave investigation of other step-sizes to future work.
\end{itemize}
See Appendix~\ref{app:sgd_bias} for a detailed proof of the theorem. 

\subsection{SGD with Data Drop is Optimal in the Agnostic Setting}\label{subsec:agn_sgd_dd}
In this section, we modify SGD so that despite having constant step size, the algorithm converges to the optimal solution as $t\rightarrow \infty$ even if the noise in each observation $\noise_t(X)$ can depend on $X$. The modified algorithm is known as SGD with data drop (\sgddd, Algorithm~\ref{alg_SGDDD}): fix $K \in \mathbb{N}$ and run SGD on samples  $X_{Kr}$ for $r \in \mathbb{N}$, and ignore the other samples. Theorem~\ref{thm:agn_sgd_dd} below shows that if $K =\Omega(\tmix \log{T})$, then the error is $O(\frac{\tmix \log T}{T})$. Combined with the lower bounds in Theorems~\ref{thm:agn_minimax} and~\ref{thm:bias-lb}, this implies that \sgddd is optimal up to log factors -- in particular, the mixing time must appear in the rates. The analysis simply bounds the distance between the iterates of SGD with independent samples and the respective iterates of \sgddd with Markovian samples.

We now formally describe the algorithm and result. Given samples from an exponentially ergodic finite state Markov Chain, $\MC$ with stationary distribution $\pi$ and mixing time $\tmix$, for $T \in \mathbb{N}$ we obtain data $(X_t,Y_t)_{t=1}^{T}$ corresponding to the states of the Markov chain $X_1 \to \cdots \to X_T \sim \MC$. We pick $K = \tmix \lceil L\log_2{T}\rceil$ for some constant $L > 0 $ to be fixed later. For the sake of simplicity we assume that $T/K$ is an integer. 

\begin{algorithm}
\caption{\sgddd}
\label{alg_SGDDD}
\begin{algorithmic}
\REQUIRE  $T \in \mathbb{N}$ , $(X_1,Y_1),\dots, (X_T,Y_T) \in  \R^d\times \R$ , step size $\alpha >0$, initial point $w_1 \in \R^d$, drop number $K \leq T$

\FOR{t in range [1, $T/K$]}
\STATE Set \begin{equation}\label{e:sgd-dd}
w_{t+1} \leftarrow w_t - \alpha X_{tK}\left(\langle w_t,X_{tK}\rangle - Y_{tK}\right)\,.
\end{equation}
\ENDFOR

\RETURN $\hat{w} \leftarrow \frac{2K}{T}\sum_{s = T/2K+2}^{T/K + 1}w_{s}\,.$
\end{algorithmic}
\end{algorithm}



We now present our theorem bounding the bias and variance for \sgddd. 
\begin{theorem}[\sgddd]\label{thm:agn_sgd_dd}
Let $MC$ be any exponentially mixing ergodic finite state Markov Chain with stationary distribution $\pi$ and mixing time $\tmix$. For $T \in \mathbb{N}$ we obtain data $(X_t,Y_t)_{t=1}^{T}$ corresponding to the states of the Markov chain $X_1 \to \cdots \to X_T \sim \MC$. Let $\alpha$ be small enough as given in Theorem 1 of \cite{jain2018parallelizing}. Then
\begin{align*}
&\mathbb{E}[\loss(\hat{w})] - \loss(w^*) \\&\quad \leq \underbrace{ \exp\left( \frac{-\alpha T}{C \cdot L\cdot  \tmix \kappa\log_2{T}}\right) \norm{w_0 - w^*}^2 + \frac{C\cdot L\cdot \tmix \mathrm{Tr}\left(A^{-1} \Sigma\right)\log_2T}{T}}_{\text{Suboptimality for i.i.d. SGD with $T/K$ samples}} + \underbrace{\frac{16\|w_0\|^2}{T^{L-2}}+ \frac{16\alpha^2\upsilon}{T^{L-3}},}_{\text{error due to leftover correlations}}\end{align*}
where $\hat{w}$ is the output of \sgddd (Algorithm~\ref{alg_SGDDD}), $A \defeq \E_{x \sim \pi}\left[xx^{\intercal}\right]$ is the data covariance matrix and $\Sigma \defeq \E_{x \sim \pi}\left[n^2 xx^{\intercal}\right]$ is the noise covariance matrix.
\end{theorem}
\textbf{Remarks}:
\begin{itemize}[leftmargin=*]
	\itemsep 0pt
	\topsep 0pt
	\parskip 0pt
	\item The bound above has two groups of terms. The first group is the error achieved by SGD on i.i.d. samples and the second group is the error due to the fact that the samples we use are only \emph{approximately} independent.
	\item With $L=5$, the error is bounded by that of SGD on i.i.d. data plus a $O(1/T^2)$ term. 
\end{itemize}
\begin{proof}[Main ideas of the proof]
	By Lemma~\ref{lem:data_drop_independence_coupling} in Section~\ref{sec:coupling_lemmas} we can couple $(\tilde{X}_{K}, \tilde{X}_{2K},\dots,\tilde{X}_{T}) \sim \pi^{\otimes (T/K)}$ to $(X_K,X_{2K},\dots,X_{T})$ such that:
	$$\mathbb{P}\left(\tilde{X}_{K},\tilde{X}_{2K},\dots,\tilde{X}_{T}) \neq (X_{K},X_{2K},\dots,X_{T})\right) \leq \tfrac{T}{K} d(K) \leq \tfrac{T}{K}  e^{-K/\tmix}.$$
	We call the data $\left(\tilde{X}_{tK},Y_{tK}(\tilde{X}_{tK})\right)$ as $(\tilde{X}_{tK},\tilde{Y}_{tK})$ for $t = 1,\dots, \frac{T}{K}$.  We replace $(X_{tK},Y_{tK})$ in the definition of \sgddd with $(\tilde{X}_{tK},\tilde{Y}_{tK})$ (with the exogenous, contextual noise $n_{tK}(\tilde{X}_{tK})$). We call the resulting iterates $\tilde{w}_t$.
	We can first show that $\mathbb{E}\|w_t -\tilde{w}_t\|^2$ is small and hence that the guarantees for SGD with i.i.d data, run for $T/K$ steps as given in \cite{jain2018parallelizing} carry over to `SGD with Data Drop' (Algorithm~\ref{alg_SGDDD}).
We refer to Appendix~\ref{app:sgd_dd} for a detailed proof.
\end{proof}

\subsection{SGD with Constant Step Size in the Independent Noise Setting is Suboptimal}
\label{subsec:minimax_sgd_constant_step_independent_noise}
In this section, we present lower bounds for SGD with constant step size and averaging in the independent noise setting. Recall that SGD with constant step size and averaging is minimax optimal in the independent sample setting. In the Markov chain setting with independent noise, while SGD with constant step size and averaging \emph{does} converge to the optimal solution (unlike in the agnostic setting, where there can be asymptotic bias (Section \ref{subsec:agnostic_SGD_bias})), the convergence rate suffers by a factor of $\tmix$. 
Let $\textrm{SGD}_{\alpha}$ be the SGD algorithm with step size $\alpha$ and tail averaging (Algorithm~\ref{alg_SGD}). For $X_1 \to \dots \to X_T \sim \MC_0$, we denote the output of $\textrm{SGD}_{\alpha}$ corresponding to the data $D_{0}(T) := (X_t,Y_t)_{t=1}^{T}$ by $\textrm{SGD}_{\alpha}(D_{0}(T))$.  We let $w_{0}^{*}$ to be the optimal parameter corresponding to the regression problem. We have the following lower bound.
\begin{theorem}\label{thm:sgd-lb}
For every $\tau_0, d \in \mathbb{N}$, there exists a finite state Markov Chain, $\MC_0$ and associated independent noise observation model (see Section \ref{subsec:problem_settings}) with points in $\R^d$, mixing time at most $\tau_0$ and $\|w_{\MC_0}^{*}\| \leq 1$.
$$ \mathbb{E}\loss_{\MC_0}(\textrm{SGD}_{\alpha}(D_{0}(T))) - \loss_{\MC_0}(w_0^{*}) \geq \big(1-o_T(1)\big)\frac{c^{\prime}\alpha\tau_0 \sigma^2 d}{T},
$$	where $c^{\prime}$ is a universal constant and $o_T(1) \to 0$ exponentially in $T$ and $\sigma^2 = \mathbb{E}n_t^2$, the variance of the noise sequence.
\end{theorem}
See Appendix~\ref{app:sgd_lb} for a complete proof. Note that this contains an extra factor of $\tau_0$ compared to the minimax rate given in Table~\ref{tab:results}.
In Section \ref{subsec:parsgd}, we provide a variant of SGD that achieves the minimax rate for this setting. 

\input{ind_psgd}
